Secure Web Objects: Building Blocks for Metaverse Interoperability and Decentralization

This position paper explores how to support the Web's evolution through an underlying data-centric approach that better matches the data-orientedness of modern and emerging applications. We revisit the original vision of the Web as a hypermedia system that supports document composability and application interoperability via name-based data access. We propose the use of secure web objects (SWO), a data-oriented communication approach that can reduce complexity, centrality, and inefficiency, particularly for collaborative and local-first applications, such as the Metaverse and other collaborative applications. SWO are named, signed, application-defined objects that are secured independently of their containers or communications channels, an approach that leverages the results from over a decade-long data-centric networking research. This approach does not require intermediation by aggregators of identity, storage, and other services that are common today. We present a brief design overview, illustrated through prototypes for two editors of shared hypermedia documents: one for 3D and one for LaTeX. We also discuss our findings and suggest a roadmap for future research.

==> discuss.tex <==
\section{Discussion}
\label{sec:discussion}

%%\begin{itemize}
%%    \item Data immutability as a fundamental concept in facilitating distributed apps
%%    \item What one can gain from using semantically meaningful identifiers
%%    \item Relationship between data names and data/security model. Should data names be (in)dependent from app names to enable cross-app data exchanges. New APIs to enable developers to work with named data, instead of REST-like calls
%%    \item Why web3, dweb are not the anSWOr. see Tim Berners-Lee talk at Web Summit 2022: https://www.cnbc.com/2022/11/04/web-inventor-tim-berners-lee-wants-us-to-ignore-web3.html
%% \end{itemize}

The vision of a data-oriented Web is based on data immutability as a fundamental, universal concept in facilitating the Web as a distributed hypermedia information system. We argue that better aligning hypermedia object models and access methods, as well as the underlying network transport,  with the inherent data-oriented structure of the actual application domains has significant advantages with respect to ease of software development (both within and outside of the ``app'' paradigm), scalable sharing and multi-destination distribution, decentralized and asynchronous communication, and data re-use.

With semantically meaningful identifiers,  interoperability can be facilitated and security properties and access control rules can be linked to domain-specific names and name prefixes. Future work is required on exploring different options for naming and data re-use. For example, data re-use should be enables across app boundaries which seems to suggest a level of indirection in naming. Such approaches would then benefits from collection concepts for file-like {\em and} dynamic objects.

Such a concept would enable different approaches for connecting distributed logic implementations. In today's Web, the client-server model has led to representational state transfer (REST) as the universal vehicle for any form of data exchange, leading to unnecessary complications for domains that do not require common state evolution on a client and a server. In a fundamentally data-oriented Web, simple data-sharing and data access could be realized more naturally, and applications could use such APIs directly, for example for publishing data or for synchronizing data sets for a distributed set of applications. APIs for publishing and for data access would be oblivious to the number of peers – because data-oriented communication has no concept of individual connections or peers. Client-server applications with robust state evolution could still be achieved through data-oriented REST approaches such as the one described in \cite{10.1145/3517212.3558089}.

This approach should not be confused with approaches that are sometimes referred to as {\em web3}\footnote{\url{https://www.cnbc.com/2022/11/04/web-inventor-tim-berners-lee-wants-us-to-ignore-web3.html}}, such as IPFS. These systems, while claiming to provide a platform for the next Web, are merely providing a (conceptually) decentralized storage platform for accessing file-like objects, which 1) is not a useful service model for any future Web, and 2) does not enable the data-oriented benefits as described here. 




==> macros.tex <==
%!TEX root = main.tex
%=========================================================

% ====== alternative commenting system (allows inline comments) ======

\hyphenchar\font=\string"7F
\hyphenation{data-oriented}

\usepackage{ifthen, xspace}

\newboolean{showcomments}
\setboolean{showcomments}{true}
\ifthenelse{\boolean{showcomments}}
{ \newcommand{\mynote}[3]{
    \protect\fbox{\bfseries\sffamily\scriptsize#1}
    {\small$\blacktriangleright$\textsf{\emph{\color{#3}{#2}}}$\blacktriangleleft$}}}
{ \newcommand{\mynote}[3]{}}

\usepackage{xcolor}
\newcommand{\ty}[1]{\mynote{Tianyuan}{#1}{blue}}
\newcommand{\lz}[1]{\mynote{Lixia}{#1}{purple}}
\newcommand{\dku}[1]{\mynote{Dirk}{#1}{teal}}
\newcommand{\jb}[1]{\mynote{Jeff}{#1}{brown}}

%  ===== formatting ======
% Abbreviations etc.
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\vs}{vs.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\ala}{ala\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\etal}{\textit{et al.}\@\xspace}
\newcommand{\eg}{\textit{e.g.,}\@\xspace}
\newcommand{\ie}{\textit{i.e.,}\@\xspace}
\newcommand{\via}{\textit{via}\@\xspace}
\newcommand{\defacto}{\textit{de facto}\@\xspace}
\newcommand\newdef[2]{\ding{118}\xspace \textsf{#1}\xspace$\bm{\rightarrow}$\xspace(#2):\xspace}

%  ===== delete copyright permission ======
\setcopyright{none}
\makeatletter
\renewcommand\@formatdoi[1]{\ignorespaces}
\makeatother
\settopmatter{printacmref=false}
\renewcommand{\footnotetextcopyrightpermission}[1]{}
\pagestyle{plain}

